3DConvCaps: 3DUnet with Convolutional Capsule Encoder for Medical Image Segmentation

Convolutional Neural Networks (CNNs) have achieved promising results in medical image segmentation. However, CNNs require lots of training data and are incapable of handling pose and deformation of objects. Furthermore, their pooling layers tend to discard important information such as positions as well as CNNs are sensitive to rotation and affine transformation. Capsule network is a recent new architecture that has achieved better robustness in part-whole representation learning by replacing pooling layers with dynamic routing and convolutional strides, which has shown potential results on popular tasks such as digit classification and object segmentation. In this paper, we propose a 3D encoder-decoder network with Convolutional Capsule Encoder (called 3DConvCaps) to learn lower-level features (short-range attention) with convolutional layers while modeling the higher-level features (long-range dependence) with capsule layers. Our experiments on multiple datasets including iSeg-2017, Hippocampus, and Cardiac demonstrate that our 3D 3DConvCaps network considerably outperforms previous capsule networks and 3D-UNets. We further conduct ablation studies of network efficiency and segmentation performance under various configurations of convolution layers and capsule layers at both contracting and expanding paths.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> author_response.tex <==
% {\fontsize{50}{60}\selectfont Foo}{\fontsize{5}{6}\selectfont bar!}
{\Large \textbf{Authors' response}}

Dear the Associate Editor and Reviewers,\\
We are thankful for the interest shown and the comments on our manuscript. We found the reviewers’ comments very helpful in improving the paper’s quality and scientific soundness. The reviewers agreed that our method provides good theoretical justification (R\#4), outperforms the previous works (R\#3), and is laid out well and easy to read (R\#4). We have read the comments carefully and provided point-by-point answers to the comments and suggestions below. The modifications in the revised manuscript are marked in yellow. We hope the revised manuscript can meet your approval.\\

\textbf{Summary of changes:}\\
\textbullet~We have rewritten the last paragraph of section \ref{sec:intro} (page 2) to make our proposed method's motivation clearer. This addresses the concern raised by R\#3.\\
\textbullet~We have added one more experiment to Table \ref{tb:ablation} (page 6) in the revised manuscript to compare our 3DConvCap network with a similar convolutional network without capsule layers. This addresses the concern raised by R\#3.\\
\textbullet~We have adjusted the figure, which is illustrated the flowchart of our 3DConvCap, (i.e. Fig. \ref{fig:network} in the revised manuscript) to illustrate the difference between our 3DConvCaps and 3D-UCaps. This addresses the concern raised by R\#4. We also adjusted a mistake in this figure. Indeed, the first capsule kernel (3D 3x3x3 Conv Capsule, Routing 3, Stride 1) in the submitted manuscript is replaced by the 3D 3x3x3 Conv Capsule, Routing 3, Stride 2 kernel in the revised manuscript.\\
\textbullet~We have fixed all minor issues suggested by the reviewers. 

\section{Reviewer 3 (R\#3)}
\noindent
\textbf{A. General Comments: }\\\\
\textbf{- Comment \#1}:\textit{The motivation, in the final part of Section I, could be improved. It is not clear that the proposal is for better efficiency, due to the reduction of the capsules in comparison with other capsule-based networks, and/or for better effectiveness in comparison with convolutional networks and other capsule-based networks. }\\\\
\textit{Response:} Thank you for your concern. Our motivation comes from the success of 3D-UCaps \cite{nguyen20213ducaps}
% (oral, MICCAI 2021)
. It has been proved by 3D-UCaps \cite{nguyen20213ducaps} that 3D-UCaps is not only a SOTA capsule-based medical image segmentation approach but also achieves competitive performance with plausible model size compared with CNN-based approaches. However, like other capsule-based approaches, inference time is a shortcoming in 3D-UCaps because of the dynamic routing procedure. Our ablation study shows that capsule blocks work effectively at high-level feature to model global relationship, whereas convolutional block is able to proficiently learn local feature. Therefore, we improve 3D-UCaps by redesigning the contracting path, which starts with convolutional blocks to capture low-level features and then capsule blocks to handle high-level features. The objectives of our proposed 3DConvCaps are two-fold: i) aims to extract better visual representation while modeling the part-whole relations; ii) reduce inference time while keep being a plausible model size. 

Therefore, in order to answer you question, our propose method is for better effectiveness in comparison with other capsule-based networks and  convolutional networks (with equivalence model complexity).

Accordingly, we have modified the last paragraph in Section \ref{sec:intro}, (page 2).\\

% \textit{{Based on the above progress, our motivation comes from the success of 3D-UCaps \mbox{\cite{nguyen20213ducaps}}
% % (oral, MICCAI 2021)
% . It has been proved by 3D-UCaps \mbox{\cite{nguyen20213ducaps}} that 3D-UCaps is not only a SOTA capsule-based medical image segmentation approach but also achieves competitive performance with plausible model size compared with CNN-based approaches. However, like other capsule-based approaches, inference time is a shortcoming in 3D-UCaps because of the dynamic routing procedure. Our ablation study shows that capsule blocks work effectively at high-level feature to model global relationship, whereas convolutional block is able to proficiently learn local feature. Therefore, we improve 3D-UCaps by redesigning the contracting path, which starts with convolutional blocks to capture low-level features and then capsule blocks to handle high-level features. The objectives of our proposed 3DConvCaps are two-fold: i) aims to extract better visual representation while modeling the part-whole relations; ii) reduce inference time while keep being a plausible model size.} The comparison between our 3DConvCaps and the existing Capsule-based MIS methods is given in Table \ref{tb:compare}.}\\
% as follows:

% \textit{Based on the above progress, our motivation comes from the success of 3D-UCaps \cite{nguyen20213ducaps}
% (oral, MICCAI 2021)
% . It has been proved by 3D-UCaps \cite{nguyen20213ducaps} that 3D-UCaps inherits the merits of capsule blocks and it outperforms other Capsule-based networks while achieving competitive results with CNN-based approaches with plausible computational complexity. However, our ablation study shows that capsule blocks work effectively at high-level feature to model global relationship, whereas convolutional block is able to proficiently learn local feature. Therefore, we improve 3D-UCaps by redesigning the contracting path, which starts with convolutional blocks to capture low-level features and then capsule blocks to handle high-level features. The comparison between our 3DConvCaps and the existing Capsule-based MIS methods is given in Table I.}
% \hl{add the first paragraph}
%, our proposed method is designed for better effectiveness in comparison with convolutional networks and other capsule-based networks with similar configurations. We have rewritten the final part of section I to make our proposal clearer. We hope that the changes can address your concern.
% We think that we have make our proposal clear in the introduction paragraphs. Indeed, in the first paragraph of introduction, we first mention about the limitations of CNN-based networks in medical imaging. Then, we point out the efficiency of capsule-based network on MIS in from line 12 - 15. 
% \\\\
\noindent
\textbf{- Comment \#2:}\textit{ Note that, since the tendency (according to the given references) is to reduce the number of capsules, to demonstrate the advantages of using capsules, and so of the proposed method, a comparison with a similar convolutional network without capsules is required. The comparison with U-Net is not valid since the hyperparameters were not the same.}
\begin{table*}[th]
\centering
\caption{Performance and network efficiency comparison on testing set of iSeg. }
\begin{tabular}{l|ccc|cc|cccc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{Encoder} & \multicolumn{2}{c|}{Decoder} & \multicolumn{4}{c|}{Performance} & \multicolumn{2}{c}{Network Efficiency}\\ \cline{2-12}
& Conv. & Cap. & Con + Cap. & Conv. & Cap. & WM & GM & CSF & Aver. & \shortstack{Time \\ Inference(s)} & \shortstack{Model \\ size}\\\hline
{3D-UNet (baseline)} & {\cmark} & {\xmark} & {\xmark} & {\cmark}& {\xmark} & {89.68}&{90.77} &{92.97} & {91.14}& {26}  &{5.8M} \\
3D-SegCaps \cite{nguyen20213ducaps} & \xmark & \cmark & \xmark & \xmark& \cmark & 71.01&73.60 &90.68 &78.43&  155 & 7.0M\\
3D-UCaps \cite{nguyen20213ducaps} &  \xmark & \cmark & \xmark & \cmark& \xmark &89.08 &90.67 & 94.54& 91.43 & 150 & 3.4M \\
\textbf{Our 3DConvCaps} &  \xmark & \xmark & \cmark & \cmark& \xmark & 92.35 &93.60 &96.09 &94.01 & 48 & 4.0M \\ \bottomrule
\end{tabular} 
\label{tb:ablation_response}
\end{table*}
\\\\
\textit{Response}: We thank the reviewer for your careful reading. We have added one more experiment to our ablation study i.e., Table 5. In this additional experiment, we replace all capsule blocks by convolutional blocks. With that setup, the network becomes 3D-UNet, which shares the same number of layers and blocks as our 3DConvCaps. The comparison between this 3D-UNet (baseline) and other 3D-Capsule-based approaches is shown in the following Table \ref{tb:ablation_response} (i.e., Table \ref{tb:ablation} in the revised manuscript). As shown in Table \ref{tb:ablation_response}, 3D-UCaps \cite{nguyen20213ducaps}, a SOTA 3D Capsule-based approach in medical image segmentation, obtains competitive results with 3D-UNet (baseline) with less model size. However, time inference consumption is a big challenge in 3D-UCaps \cite{nguyen20213ducaps} because of dynamic routing. Compared to 3D-UNet (baseline), our 3DConvCap yields a substantial margin on performance while keeping model size smaller and time inference plausible. Compare to the SOTA 3D Capsule-based approach, 3D-UCaps \cite{nguyen20213ducaps}, our network not only outperforms on all three classes of WM, GM, CSF but also requires less time inference with competitive model size. 

We have added this additional experiment in the revised manuscript at Table \ref{tb:ablation}. We also updated experiment analysis at the last paragraph of subsection \ref{subsec:performance}\\\\
%the comparison with the similar convolutional network in the ablation study table (Table V in the revised manuscript or Table \ref{tb:ablation} in this author's response letter). Indeed, inspired from \cite{cciccek20163d}, we implement the 3D-UNet, equivalent to our 3DConvCaps in terms of model structure and layer depths, by replacing the last two capsule layers of our 3DConvCaps with two alternative convolutional layers.
%As illustrated in Table \ref{tb:ablation}, our method shows efficiency by leveraging both CNN layers and capsule layers for short-range and long-range information, respectively. Indeed, 3DConvCaps outperforms other methods by performance. In addition, our method has acceptable time inference, compared to the fastest one 3D-UNet (i.e. 48s v.s. 26s), and has a comparable model size, in comparison with the smallest one 3D-UCaps (i.e. 4.0M v.s. 3.4M).\\
% \indent
% We also have added related writing in the last paragraph of section IV in the revised manuscript. We hope that these supplements can address your concern.
\textbf{B. Specific Comments:}\\\\
We thank the reviewer for careful reading. We apologize for our shortcomings in the manuscript. We have updated our revised manuscript regarding specific comments as follows:  
%Below are our modifications on each issue from your specific comments.\\\\


\textbullet~\textit{Multi-SegCaps citation and appearance}: We have fixed its citation and appearance in paragraph 2, section \ref{sec:intro}, in the revised manuscript.


\textbullet~\textit{Line 12, Second paragraph, Section 1: Reference [16] is related to classification and not to segmentation. Nearby in the subsequent lines: is better performance $\rightarrow$ has better performance. ... missing temporal information: it requires a reference here.}: In the second paragraph, section \ref{sec:intro} of the submitted manuscript, we have rewritten lines from 10 - 16 to address your concern. It now becomes lines 10 - 18, paragraph 2, section \ref{sec:intro}, in the revised manuscript. Indeed, the reference [16] now becomes the reference \cite{jimenez2018capsule} in the revised manuscript. This reference points out the advantage of a capsule network on small amounts of annotated data and class-imbalanced data.
% \hl{need to revise the line number before submitting}  


\textbullet~\textit{Related works and introduction are very similar.}: We would like to clarify the difference between the introduction and related works. The introduction aims to provide the pros and cons of two approaches i.e. convolutional-based approaches with capsule-based approaches. Herein, we also introduce our motivation which is inspired by 3D-UCaps \cite{nguyen20213ducaps} at the end of the introduction. The related works section provides more technical details of existing works in both convolutional-based approaches and capsule-based approaches. We have rewritten the last paragraph of the introduction to reinforce the advantage of our proposal.

\textbullet~ Time consumption: We have updated Table 5 in the revised manuscript with inference time consumption and model size. 



%\textbullet~Section $III$: We have fixed the mentioned grammar.\\


% \textbullet~Inference time consumption: In section $III$-B, we have rewritten the sentence following your suggestion. We also added a reference, which is Table V, to reinforce our statement that Capsule-based MIS is time-consuming when it comes to inference.\\


% \textbullet~Section $III$-B (b): We have fixed the last layer capsule's shape from $H \times W \times D \times C \times A$ to $H/8 \times W/8 \times D/8 \times C \times A$.\\


\textbullet~Machine configuration: We have added mode details regarding machine configuration. The CPU and GPU models are Intel(R) Core(TM) i9-9920X CPU \@ 3.50GHz and GeForce RTX 2080 Ti, respectively.


\textbullet~ Typos, grammars: Thank you for your careful reading. We have fixed them in the revised manuscript according to your suggestion.
% \textbullet~The citation [48] now becomes citation [14] and is first mentioned in paragraph 2, section I in the revised manuscript.

\section{Reviewer 4 (R\#4)}
\noindent
\textbf{Issues to Address in the Rebuttal:}\\
- \textbf{Comment \#1}: \textit{The architectural differences between the 3DUCaps and
3DConvCaps encoder need to be more obvious.}

\textit{Response}: We have adjusted the figure \ref{fig:network} in the revised manuscript, which illustrates the flowchart of our 3DConvCaps. In the revised manuscript, we have partitioned the contracting path into 2 parts corresponding to convolutional blocks and capsule blocks by two different colors.

We also added an additional figure in this response to illustrate the difference between our 3DConvCaps and 3DUCaps as in Fig \ref{fig:diff}.
\begin{figure}[!t]
	\centering
	%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
	\includegraphics[width=.9\linewidth]{ICPR2022-SSL-MIS/Figs/3dconvcaps_revised-Difference.pdf}
	\caption{Difference between 3DUCaps and 3DConvCaps}
	%\label{fig:model}
	\label{fig:diff}
	\vspace{-0.3cm}
\end{figure}
\\
%to illustrate the difference between our 3DConvCaps and 3D-UCaps. Indeed, we illustrate the CNN-based encoder feature map and the capsule-based encoder feature map with different colors. We hope that our revised illustration of 3DConvCaps can address your concern.

\noindent
- \textbf{Comment \#2}: \textit{Include the model of the RTX GPU used.}

\textit{Response:} We have added more details of machine specifications to the revised manuscript. Namely, the CPU and GPU models are Intel(R) Core(TM) i9-9920X CPU \@ 3.50GHz and GeForce RTX 2080 Ti, respectively.
%CPU and GPU models in Section IV (d) of the revised manuscript. The CPU and GPU models are Intel(R) Core(TM) i9-9920X CPU \@ 3.50GHz and GeForce RTX 2080 Ti, respectively.
